Enhancing Pretrained Model-based Continual Representation Learning via Guided Random Projection

Recent paradigms in Random Projection Layer (RPL)-based continual representation learning have demonstrated superior performance when building upon a pre-trained model (PTM). These methods insert a randomly initialized RPL after a PTM to enhance feature representation in the initial stage. Subsequently, a linear classification head is used for analytic updates in the continual learning stage. However, under severe domain gaps between pre-trained representations and target domains, a randomly initialized RPL exhibits limited expressivity under large domain shifts. While largely scaling up the RPL dimension can improve expressivity, it also induces an ill-conditioned feature matrix, thereby destabilizing the recursive analytic updates of the linear head. To this end, we propose the Stochastic Continual Learner with MemoryGuard Supervisory Mechanism (SCL-MGSM). Unlike random initialization, MGSM constructs the projection layer via a principled, data-guided mechanism that progressively selects target-aligned random bases to adapt the PTM representation to downstream tasks. This facilitates the construction of a compact yet expressive RPL while improving the numerical stability of analytic updates. Extensive experiments on multiple exemplar-free Class Incremental Learning (CIL) benchmarks demonstrate that SCL-MGSM achieves superior performance compared to state-of-the-art methods.

==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

% 这是一个包含多种元素的示例章节


% 示例图片 - 双栏宽度
\begin{figure*}[!tb]
\centering
\includegraphics[width=0.9\linewidth]{figures/content/example_figure.pdf}
\caption{\textbf{Example figure with full-width layout.} This demonstrates how to include a figure that spans both columns in a two-column layout. Replace this placeholder with your actual figure. The figure should be in PDF format for vector graphics to ensure high quality and scalability.}
\label{fig:example}
\end{figure*}

% 段落 1: 背景和动机
Recent advances in [your research field] have significantly transformed [the application domain]~\cite{example2023paper}. Despite impressive progress in [specific aspect], several fundamental challenges remain unaddressed. In particular, [describe the main problem] requires a comprehensive understanding of [key factors] and careful consideration of [important constraints].

% 段落 2: 现有方法的局限性
Prior work has explored various approaches to tackle this problem~\cite{smith2022method, johnson2023approach}. However, existing methods exhibit clear limitations when applied to [specific scenarios]:

\begin{itemize}
\item \textbf{First limitation}: [Describe the first major limitation]. For example, traditional approaches typically [describe behavior] while [describe the actual requirement].

\item \textbf{Second limitation}: [Describe the second limitation]. This results in [negative consequences] and prevents [desired outcomes].

\item \textbf{Third limitation}: [Describe the third limitation]. The lack of [missing component] leads to [specific problems] in [particular contexts].
\end{itemize}

% 段落 3: 我们的解决方案
In this work, we address these challenges by proposing \textbf{YourMethodName}, a novel framework that [high-level description of your approach]. Our key insight is that [describe your key insight or observation]. Specifically, we introduce [list your main technical contributions] to achieve [your goals].

% 段落 4: 主要贡献
The main contributions of this paper are summarized as follows:

\begin{itemize}
\item We propose [first contribution], which enables [benefit or capability].

\item We introduce [second contribution], providing [advantage] and addressing [specific problem].

\item We develop [third contribution], yielding [improved performance or new capability].

\item We conduct comprehensive experiments on [datasets/benchmarks], demonstrating that our method achieves [performance improvements] compared to state-of-the-art approaches.
\end{itemize}

% 示例数学公式
As illustrated in Equation~\ref{eq:example}, our approach can be formalized as:
\begin{equation}
\label{eq:example}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \lambda \mathcal{L}_{\text{reg}}
\end{equation}
where $\mathcal{L}_{\text{task}}$ represents the task-specific loss, $\mathcal{L}_{\text{reg}}$ is the regularization term, and $\lambda$ controls the trade-off between the two objectives.

% 段落 5: 论文组织结构
The remainder of this paper is organized as follows. Section~\ref{sec:related} reviews related work in [relevant areas]. Section~\ref{sec:method} presents our proposed method in detail. Section~\ref{sec:experiments} describes our experimental setup and reports comprehensive results. Finally, Section~\ref{sec:conclusion} concludes the paper and discusses future directions.


==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related}

% 本章节展示如何组织相关工作，包含多个子主题

% 子主题 1
\subsection{[First Research Area]}
\label{subsec:area1}

Early work in [first research area] primarily focused on [early approaches]~\cite{author2020early}. These methods typically relied on [key techniques or assumptions] and achieved [certain results]. For instance, [Author et al.]~\cite{author2021specific} proposed [method name], which [description]. However, this approach was limited by [limitations].

More recent advances have explored [newer directions]~\cite{recent2023work}. [Describe recent developments and their contributions]. Despite these improvements, [remaining challenges or gaps] continue to pose significant obstacles.

% 子主题 2
\subsection{[Second Research Area]}
\label{subsec:area2}

% 示例表格 - 比较不同方法
\begin{table}[t]
\centering
\caption{Comparison of different approaches in [research area]. This table summarizes the key characteristics and limitations of existing methods.}
\label{tab:comparison}
\tablestyle{4pt}{1.2}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Feature A} & \textbf{Feature B} & \textbf{Limitation} \\
\midrule
Method 1~\cite{example2023paper} & \checkmark & \texttimes & Limited scalability \\
Method 2~\cite{smith2022method} & \checkmark & \checkmark & High complexity \\
Method 3~\cite{johnson2023approach} & \texttimes & \checkmark & Poor generalization \\
\textbf{Ours} & \checkmark & \checkmark & -- \\
\bottomrule
\end{tabular}
\end{table}

Another line of research has investigated [second research area]~\cite{baseline2022paper}. [Describe this research direction and its relevance to your work]. As shown in Table~\ref{tab:comparison}, existing methods differ in [key aspects]. While [Method X]~\cite{methodx2023} achieves [certain advantages], it suffers from [specific drawbacks]. Similarly, [Method Y]~\cite{methody2022} addresses [problem A] but fails to handle [problem B].

% 子主题 3
\subsection{[Third Research Area]}
\label{subsec:area3}

The integration of [concept A] with [concept B] has gained increasing attention in recent years~\cite{integration2023}. [Describe this integration and why it matters]. Several notable works have made progress in this direction:

\begin{itemize}
\item \textbf{[Work 1]}~\cite{work1}: [Brief description of contribution and limitation]
\item \textbf{[Work 2]}~\cite{work2}: [Brief description of contribution and limitation]
\item \textbf{[Work 3]}~\cite{work3}: [Brief description of contribution and limitation]
\end{itemize}

% 子主题 4: 与本文工作的关系
\subsection{Relation to Our Work}
\label{subsec:relation}

Our work is most closely related to [specific area or methods]~\cite{close2023work}. However, we differ in several key aspects. First, unlike [previous approach], our method [describe key difference 1]. Second, we introduce [novel component], which enables [capability not available before]. Third, our framework [describe architectural or methodological difference].

Furthermore, while prior work has primarily focused on [narrow scope], we provide a more comprehensive solution that addresses [broader challenges]. The experimental results in Section~\ref{sec:experiments} demonstrate that our approach achieves significant improvements over these existing methods.


==> sections/3_method.tex <==
\section{Method}
\label{sec:method}

% 本章节展示技术方法，包含算法、公式、架构图等

In this section, we present the details of our proposed method. We first provide an overview of the framework architecture in Section~\ref{subsec:overview}, followed by detailed descriptions of the key components in Sections~\ref{subsec:component1}--\ref{subsec:component3}.

% 方法概述
\subsection{Overview}
\label{subsec:overview}

% 示例架构图
\begin{figure*}[!tb]
\centering
\includegraphics[width=0.95\linewidth]{figures/content/architecture.pdf}
\caption{\textbf{Overview of our proposed framework.} The architecture consists of three main components: (a) [Component 1] for [purpose], (b) [Component 2] for [purpose], and (c) [Component 3] for [purpose]. The data flows from left to right, with [describe the processing pipeline].}
\label{fig:architecture}
\end{figure*}

As illustrated in Figure~\ref{fig:architecture}, our framework takes [input description] and produces [output description] through [number] main stages. The overall objective can be formulated as:

\begin{equation}
\label{eq:objective}
\min_{\theta} \mathbb{E}_{(x,y) \sim \mathcal{D}} \left[ \ell(f_\theta(x), y) \right] + \Omega(\theta)
\end{equation}

where $\theta$ denotes the model parameters, $\mathcal{D}$ is the data distribution, $f_\theta$ is our model, $\ell$ is the loss function, and $\Omega(\theta)$ represents the regularization term.

% 第一个组件
\subsection{[Component 1 Name]}
\label{subsec:component1}

The first component of our framework is designed to [purpose and motivation]. Given an input $\mathbf{x} \in \mathbb{R}^{d}$, we first apply [transformation]:

\begin{equation}
\label{eq:component1}
\mathbf{h} = \text{Encoder}(\mathbf{x}) = \mathbf{W}_e \mathbf{x} + \mathbf{b}_e
\end{equation}

where $\mathbf{W}_e \in \mathbb{R}^{d_h \times d}$ and $\mathbf{b}_e \in \mathbb{R}^{d_h}$ are learnable parameters. The resulting representation $\mathbf{h}$ captures [what it captures].

To enhance [specific aspect], we introduce [novel mechanism]:

\begin{equation}
\label{eq:attention}
\alpha_{ij} = \frac{\exp(\text{score}(\mathbf{h}_i, \mathbf{h}_j))}{\sum_{k=1}^{n} \exp(\text{score}(\mathbf{h}_i, \mathbf{h}_k))}
\end{equation}

where $\text{score}(\cdot, \cdot)$ measures the compatibility between different representations.

% 第二个组件
\subsection{[Component 2 Name]}
\label{subsec:component2}

% 示例算法伪代码
\begin{algorithm}[t]
\caption{[Algorithm Name]}
\label{alg:main}
\begin{algorithmic}[1]
\Require Input data $\mathbf{X} = \{\mathbf{x}_1, \ldots, \mathbf{x}_n\}$, hyperparameters $\lambda, \eta$
\Ensure Output predictions $\mathbf{Y} = \{\mathbf{y}_1, \ldots, \mathbf{y}_n\}$
\State Initialize parameters $\theta \leftarrow \theta_0$
\For{$t = 1$ to $T$}
    \State Sample mini-batch $\mathcal{B} \subset \{1, \ldots, n\}$
    \For{$i \in \mathcal{B}$}
        \State Compute forward pass: $\hat{\mathbf{y}}_i = f_\theta(\mathbf{x}_i)$
        \State Compute loss: $\mathcal{L}_i = \ell(\hat{\mathbf{y}}_i, \mathbf{y}_i)$
    \EndFor
    \State Compute gradient: $\nabla_\theta \mathcal{L} = \frac{1}{|\mathcal{B}|} \sum_{i \in \mathcal{B}} \nabla_\theta \mathcal{L}_i$
    \State Update parameters: $\theta \leftarrow \theta - \eta \nabla_\theta \mathcal{L}$
\EndFor
\State \Return $\mathbf{Y} = \{f_\theta(\mathbf{x}_i)\}_{i=1}^{n}$
\end{algorithmic}
\end{algorithm}

Building on the representations from the previous component, we design [Component 2] to [purpose]. The complete procedure is summarized in Algorithm~\ref{alg:main}. The key idea is to [describe key idea] by iteratively [describe iteration process].

At each step $t$, we update [what gets updated] according to:

\begin{equation}
\label{eq:update}
\mathbf{z}^{(t+1)} = \mathbf{z}^{(t)} + \alpha \cdot \nabla_{\mathbf{z}} \mathcal{F}(\mathbf{z}^{(t)}, \mathbf{h})
\end{equation}

where $\mathcal{F}$ is an energy function and $\alpha$ is the step size.

% 第三个组件
\subsection{[Component 3 Name]}
\label{subsec:component3}

% 子图示例
\begin{figure}[!tb]
\centering
\begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/content/sub_figure_a.pdf}
    \caption{Visualization of [aspect A]}
    \label{fig:sub_a}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/content/sub_figure_b.pdf}
    \caption{Visualization of [aspect B]}
    \label{fig:sub_b}
\end{subfigure}
\caption{\textbf{Detailed visualization of [component].} (a) shows [description of subplot a], while (b) illustrates [description of subplot b]. These visualizations demonstrate [what they demonstrate].}
\label{fig:visualization}
\end{figure}

The final component integrates outputs from the previous stages to produce the final prediction. As shown in Figure~\ref{fig:visualization}, [describe what the figure shows]. Mathematically, this can be expressed as:

\begin{equation}
\label{eq:final}
\hat{\mathbf{y}} = g(\mathbf{z}, \mathbf{h}) = \text{Decoder}(\mathbf{z} \oplus \mathbf{h})
\end{equation}

where $\oplus$ denotes the fusion operation and $g$ is the final prediction function.

% 损失函数
\subsection{Training Objective}
\label{subsec:training}

To train our model end-to-end, we define a multi-task loss function that combines [different objectives]:

\begin{equation}
\label{eq:total_loss}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{pred}} + \lambda_1 \mathcal{L}_{\text{aux}} + \lambda_2 \mathcal{L}_{\text{reg}}
\end{equation}

where:
\begin{itemize}
\item $\mathcal{L}_{\text{pred}}$ is the main prediction loss, typically defined as:
\begin{equation}
\mathcal{L}_{\text{pred}} = \frac{1}{N} \sum_{i=1}^{N} \|\hat{\mathbf{y}}_i - \mathbf{y}_i\|^2
\end{equation}

\item $\mathcal{L}_{\text{aux}}$ is an auxiliary loss that encourages [specific property]

\item $\mathcal{L}_{\text{reg}}$ is a regularization term to prevent overfitting

\item $\lambda_1, \lambda_2$ are hyperparameters that balance the different objectives
\end{itemize}

% 实现细节
\subsection{Implementation Details}
\label{subsec:implementation}

We implement our framework using [framework name, \eg PyTorch]. The model is trained for [number] epochs with batch size [size] using the Adam optimizer~\cite{kingma2014adam} with learning rate [lr]. We employ [specific techniques like dropout, batch normalization, etc.] to improve training stability and generalization. All experiments are conducted on [hardware specifications].


==> sections/4_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

% 本章节展示实验设置和结果，包含多种类型的表格和图表

In this section, we evaluate our proposed method through comprehensive experiments. We first describe the experimental setup in Section~\ref{subsec:setup}, followed by quantitative results in Section~\ref{subsec:quantitative} and qualitative analysis in Section~\ref{subsec:qualitative}. Finally, we present ablation studies in Section~\ref{subsec:ablation}.

% 实验设置
\subsection{Experimental Setup}
\label{subsec:setup}

\paragraph{Datasets}
We evaluate our method on [number] widely-used benchmarks:
\begin{itemize}
\item \textbf{Dataset 1}~\cite{dataset1}: Contains [number] samples with [characteristics]. We follow the standard split of [train/val/test].
\item \textbf{Dataset 2}~\cite{dataset2}: A challenging dataset featuring [characteristics]. We use [number] samples for training and [number] for testing.
\item \textbf{Dataset 3}~\cite{dataset3}: Designed for [specific task], consisting of [description].
\end{itemize}

\paragraph{Evaluation Metrics}
Following prior work~\cite{baseline2022paper}, we use the following metrics:
\begin{itemize}
\item \textbf{Metric 1}: Measures [what it measures]
\item \textbf{Metric 2}: Evaluates [what it evaluates]
\item \textbf{Metric 3}: Quantifies [what it quantifies]
\end{itemize}

\paragraph{Baselines}
We compare our method against several state-of-the-art approaches:
\begin{itemize}
\item \textbf{Method A}~\cite{methoda}: [Brief description]
\item \textbf{Method B}~\cite{methodb}: [Brief description]
\item \textbf{Method C}~\cite{methodc}: [Brief description]
\item \textbf{Method D}~\cite{methodd}: [Brief description]
\end{itemize}

\paragraph{Implementation Details}
We implement our method using PyTorch and train on 4 NVIDIA A100 GPUs. The model is optimized using AdamW with a learning rate of $2 \times 10^{-4}$ and weight decay of $0.01$. We train for 100 epochs with batch size 32. Data augmentation includes random cropping, horizontal flipping, and color jittering.

% 定量结果
\subsection{Quantitative Results}
\label{subsec:quantitative}

% 主要结果表格
\begin{table*}[t]
\centering
\caption{Quantitative comparison on three benchmarks. Best results are in \textbf{bold}, and second best are \underline{underlined}. $\uparrow$ indicates higher is better, $\downarrow$ indicates lower is better.}
\label{tab:main_results}
\tablestyle{6pt}{1.3}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Dataset 1}} & \multicolumn{3}{c|}{\textbf{Dataset 2}} & \multicolumn{3}{c}{\textbf{Dataset 3}} \\
& Metric1$\uparrow$ & Metric2$\uparrow$ & Metric3$\downarrow$ & Metric1$\uparrow$ & Metric2$\uparrow$ & Metric3$\downarrow$ & Metric1$\uparrow$ & Metric2$\uparrow$ & Metric3$\downarrow$ \\
\midrule
Method A~\cite{methoda} & 72.3 & 68.5 & 0.245 & 65.8 & 62.1 & 0.312 & 70.2 & 66.8 & 0.278 \\
Method B~\cite{methodb} & 75.6 & 71.2 & 0.223 & 68.4 & 65.3 & 0.289 & 73.5 & 69.7 & 0.251 \\
Method C~\cite{methodc} & 78.1 & 73.8 & 0.208 & 71.2 & 68.6 & 0.267 & 76.3 & 72.4 & 0.234 \\
Method D~\cite{methodd} & \underline{80.5} & \underline{76.3} & \underline{0.195} & \underline{74.6} & \underline{71.2} & \underline{0.248} & \underline{79.1} & \underline{75.6} & \underline{0.219} \\
\midrule
\textbf{Ours} & \textbf{83.7} & \textbf{79.8} & \textbf{0.178} & \textbf{77.9} & \textbf{74.5} & \textbf{0.231} & \textbf{82.4} & \textbf{78.9} & \textbf{0.203} \\
\bottomrule
\end{tabular}
\end{table*}

Table~\ref{tab:main_results} presents the quantitative comparison on three benchmarks. Our method consistently outperforms all baselines across all datasets and metrics. Specifically, compared to the best baseline (Method D), our approach achieves:
\begin{itemize}
\item \textbf{Dataset 1}: +3.2\% on Metric1, +3.5\% on Metric2, and -8.7\% on Metric3
\item \textbf{Dataset 2}: +3.3\% on Metric1, +3.3\% on Metric2, and -6.9\% on Metric3
\item \textbf{Dataset 3}: +3.3\% on Metric1, +3.3\% on Metric2, and -7.3\% on Metric3
\end{itemize}

These improvements demonstrate the effectiveness of our proposed components, particularly [Component X] which addresses [specific limitation of baselines].

% 不同设置下的结果
\begin{table}[t]
\centering
\caption{Performance under different settings on Dataset 1. Our method maintains robust performance across various conditions.}
\label{tab:different_settings}
\tablestyle{4pt}{1.2}
\begin{tabular}{lcccc}
\toprule
\textbf{Setting} & \textbf{Baseline} & \textbf{Method D} & \textbf{Ours} & \textbf{Gain} \\
\midrule
Standard & 75.6 & 80.5 & \textbf{83.7} & +3.2 \\
Low-resource & 68.2 & 72.8 & \textbf{76.4} & +3.6 \\
High-noise & 62.5 & 67.3 & \textbf{71.1} & +3.8 \\
Cross-domain & 58.9 & 63.7 & \textbf{68.2} & +4.5 \\
\bottomrule
\end{tabular}
\end{table}

% 定性结果
\subsection{Qualitative Results}
\label{subsec:qualitative}

% 示例比较图
\begin{figure*}[!tb]
\centering
\includegraphics[width=\linewidth]{figures/content/qualitative_comparison.pdf}
\caption{\textbf{Qualitative comparison with baseline methods.} From left to right: Input, Ground Truth, Method B, Method D, and Ours. Our method produces results that are more [describe advantages], particularly in [challenging scenarios]. Red boxes highlight regions where our method shows significant improvements.}
\label{fig:qualitative}
\end{figure*}

Figure~\ref{fig:qualitative} shows qualitative comparisons between our method and baselines. As can be observed, our approach generates more [quality attribute] results, especially in challenging cases involving [difficult scenarios]. While Method D performs reasonably well in [certain aspects], it struggles with [specific challenges]. In contrast, our method successfully handles these cases by [explain why your method works].

% 消融实验
\subsection{Ablation Study}
\label{subsec:ablation}

% 消融实验表格
\begin{table}[t]
\centering
\caption{Ablation study on Dataset 1. Each row removes one component from the full model to analyze its contribution.}
\label{tab:ablation}
\tablestyle{4pt}{1.2}
\begin{tabular}{lccc}
\toprule
\textbf{Variant} & \textbf{Metric1$\uparrow$} & \textbf{Metric2$\uparrow$} & \textbf{Metric3$\downarrow$} \\
\midrule
Full Model & \textbf{83.7} & \textbf{79.8} & \textbf{0.178} \\
\midrule
w/o Component 1 & 79.2 & 75.4 & 0.201 \\
w/o Component 2 & 80.8 & 77.1 & 0.189 \\
w/o Component 3 & 81.5 & 78.2 & 0.184 \\
w/o Loss Term 1 & 82.1 & 78.6 & 0.182 \\
w/o Loss Term 2 & 82.9 & 79.2 & 0.180 \\
\bottomrule
\end{tabular}
\end{table}

To validate the effectiveness of each component, we conduct ablation studies by removing individual components from the full model. As shown in Table~\ref{tab:ablation}, each component contributes to the overall performance:

\begin{itemize}
\item \textbf{Component 1} has the largest impact (-4.5\% on Metric1), confirming its importance for [its role].
\item \textbf{Component 2} contributes -2.9\% on Metric1, demonstrating its value in [its purpose].
\item \textbf{Component 3} provides -2.2\% improvement, showing that [its benefit].
\item Both loss terms contribute to performance, with Loss Term 1 being more critical.
\end{itemize}

% 超参数分析
\subsection{Hyperparameter Analysis}
\label{subsec:hyperparameter}

\begin{figure}[!tb]
\centering
\includegraphics[width=0.9\linewidth]{figures/content/hyperparameter_analysis.pdf}
\caption{\textbf{Impact of key hyperparameters.} We analyze the effect of (left) $\lambda_1$ and (right) $\lambda_2$ on performance. The model is relatively robust to hyperparameter choices within reasonable ranges.}
\label{fig:hyperparameter}
\end{figure}

We analyze the sensitivity of our method to key hyperparameters. As shown in Figure~\ref{fig:hyperparameter}, performance is relatively stable across a wide range of $\lambda_1$ and $\lambda_2$ values, indicating that our method is robust and does not require extensive hyperparameter tuning. The optimal performance is achieved when $\lambda_1 = 0.1$ and $\lambda_2 = 0.5$.


==> sections/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% 本章节总结全文并讨论未来工作

\textcolor{red}{
\textbf{Wish everyone in VisionXLab that all the papers will be accepted for publication!}
}

In this paper, we have presented \textbf{[YourMethodName]}, a novel framework for [main task/problem]. Our key contributions include:

\begin{itemize}
\item A [describe first contribution] that enables [benefit]
\item A [describe second contribution] that addresses [limitation]
\item A [describe third contribution] that improves [aspect]
\end{itemize}

Through comprehensive experiments on [number] benchmark datasets, we have demonstrated that our method significantly outperforms existing state-of-the-art approaches. Specifically, our approach achieves [X\%] improvement on [metric] while maintaining [desirable property]. The ablation studies confirm that each component of our framework contributes meaningfully to the overall performance.

% 局限性
\subsection{Limitations}
\label{subsec:limitations}

Despite the promising results, our method has several limitations that warrant future investigation:

\begin{itemize}
\item \textbf{Computational Cost}: The current implementation requires [computational resources], which may limit its applicability to [certain scenarios]. Future work could explore more efficient architectures or approximation techniques to reduce computational requirements.

\item \textbf{Data Requirements}: Our method benefits from large-scale training data. In low-resource settings, performance may degrade. Investigating few-shot learning or transfer learning approaches could help address this limitation.

\item \textbf{Specific Scenarios}: While our method performs well on the tested benchmarks, it may struggle with [specific challenging cases]. Further research is needed to enhance robustness in these scenarios.
\end{itemize}

% 未来工作
\subsection{Future Directions}
\label{subsec:future}

Several promising directions for future research include:

\begin{itemize}
\item \textbf{Extension to Other Domains}: While we have focused on [current domain], the proposed framework is general and could potentially be applied to [other domains such as X, Y, Z]. Exploring these applications could reveal new insights and broaden the impact of our work.

\item \textbf{Integration with [Technique X]}: Recent advances in [related technique] suggest potential synergies with our approach. Investigating how to effectively combine these methods could lead to further performance improvements.

\item \textbf{Real-world Deployment}: Transitioning from research prototypes to practical systems requires addressing additional challenges such as [deployment challenges]. Future work should focus on [specific aspects] to enable real-world applications.

\item \textbf{Theoretical Analysis}: While our empirical results are strong, a deeper theoretical understanding of [why the method works] would be valuable. Developing formal guarantees or convergence proofs could strengthen the foundation of our approach.
\end{itemize}

% 总结
In conclusion, this work represents a significant step forward in [research area] by introducing [main innovation]. We hope that our contributions will inspire future research and facilitate progress toward [ultimate goal]. The code and models will be made publicly available to support reproducibility and further development by the research community.

% 致谢（如果需要可以添加）
% \section*{Acknowledgments}
% We thank [people/organizations] for [their contributions]. This work was supported by [funding sources].

